Object-centric Cross-modal Feature Distillation for Event-based Object Detection

Event cameras are gaining popularity due to their unique properties, such as their low latency and high dynamic range. One task where these benefits can be crucial is real-time object detection. However, RGB detectors still outperform event-based detectors due to the sparsity of the event data and missing visual details. In this paper, we develop a novel knowledge distillation approach to shrink the performance gap between these two modalities. To this end, we propose a cross-modality object detection distillation method that by design can focus on regions where the knowledge distillation works best. We achieve this by using an object-centric slot attention mechanism that can iteratively decouple features maps into object-centric features and corresponding pixel-features used for distillation. We evaluate our novel distillation approach on a synthetic and a real event dataset with aligned grayscale images as a teacher modality. We show that object-centric distillation allows to significantly improve the performance of the event-based student object detector, nearly halving the performance gap with respect to the teacher.

==> figures/teaser.tex <==
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=1.0\linewidth]{images/teaser.png}  
\end{center}
\vspace{-0.45cm}
\caption{(c) Visualization of the spatial heat maps of the largest scale FPN feature in the YOLOX detector \cite{ge2021yolox} using grayscale image and event frame as inputs, revealing significant differences in feature distributions with grayscale images and event frames as input. With our distillation model, foreground features are enhanced and background noise (lane markings) is weakened.}
\vspace{-0.9em}
\label{fig:teaser}
\end{figure}

==> figures/training_process.tex <==
\begin{figure}[h]
\centering 
\scalebox{0.8}{
\begin{tikzpicture}

\begin{axis}[
    % axis lines = left,
    xlabel=Epoch, 
    ylabel=AP, 
    % tick align=outside, %刻度在外显式
    % legend pos=outer south east
    legend style={at={(0.7,0.3)},anchor=north} %图例在图下方显示
    ]

% first line
\addplot[smooth,black] plot coordinates { 
(0,6.69497633)
(1,22.48297882)
(2,37.88008881)
(3,47.80266953)
(4,51.40914536)
(5,53.13244247)
(6,54.22544479)
(7,54.95412064)
(8,54.69216919)
(9,55.11352539)
(10,54.38426971)
(11,54.62501526)
(12,55.20703125)
(13,54.92284393)
(14,55.71556854)
(15,53.33985519)
(16,54.99555969)
(17,55.04685593)
(18,52.15941238)
(19,53.83487701)
(20,51.73726654)
(21,52.46629715)
(22,53.09399414)
(23,53.28549576)
(24,52.19607544)
(25,50.74947739)
(26,52.22091675)
(27,52.79984283)
(28,49.43661118)
(29,51.70531845)
(30,52.2919693)
(31,51.36697388)
(32,51.67201996)
(33,49.91793442)
(34,49.94181442)
(35,52.00580215)
};
\addlegendentry{Grayscale}

%second line
\addplot[smooth,blue] plot coordinates {
(0,0)
(1,0)
(2,4.755392551)
(3,14.4420681)
(4,25.9529171)
(5,33.13326645)
(6,35.56007767)
(7,38.51645279)
(8,38.40179062)
(9,38.4980011)
(10,39.48110199)
(11,41.06628418)
(12,42.0476532)
(13,40.22013474)
(14,40.70133209)
(15,40.32563782)
(16,39.97257614)
(17,42.08324432)
(18,39.38499451)
(19,40.05054474)
(20,38.94573975)
(21,38.89889526)
(22,42.20821381)
(23,41.66225052)
(24,40.98538589)
(25,40.22208786)
(26,39.83964157)
(27,38.12949753)
(28,41.45674133)
(29,39.7594223)
(30,42.05833054)
(31,42.77006149)
(32,42.16741562)
(33,39.0929985)
(34,39.37804794)
(35,41.0705719)
};
\addlegendentry{Event}

%third line
\addplot[smooth,red] plot coordinates {
(0,0)
(1,0)
(2,4.792881012)
(3,13.41563892)
(4,25.34893799)
(5,33.64430237)
(6,32.28922272)
(7,38.57190704)
(8,39.16532135)
(9,40.96649933)
(10,41.06422424)
(11,44.35945129)
(12,43.53496552)
(13,43.40804291)
(14,42.55268097)
(15,42.3919487)
(16,42.54895401)
(17,44.45452118)
(18,42.89054489)
(19,43.13859177)
(20,43.08556747)
(21,43.32436752)
(22,43.97312927)
(23,43.59745026)
(24,43.78784943)
(25,43.88326263)
(26,43.26064301)
(27,40.60699463)
(28,42.12292099)
(29,43.57151794)
(30,43.301754)
(31,43.51300049)
(32,44.46409607)
(33,42.64919662)
(34,41.55125809)
(35,43.4333725)
};
\addlegendentry{Event+Distillation}

\end{axis}
\end{tikzpicture}
}
\caption{The AP of pedestrian detection at the initial stage of training for grayscale-based object detection, as well as for event-based object detection training with and without feature distillation.}
\label{fig:training}
\end{figure}

==> figures/vis_perobject_attn.tex <==
\begin{figure*}[ht]
\centering
\scalebox{0.9}{
\begin{tabular}{ccccc}
% & Input    &Heat Map\\
% \includegraphics[width=0.25\textwidth]
% {images/img_000390.png} &
\rotatebox{90}{~~~~~~Grayscale} &\includegraphics[width=0.21\textwidth]{images/perobject_attn/GS_10_0_0_with_attention.jpg}&
\includegraphics[width=0.21\textwidth]{images/perobject_attn/GS_10_0_1_with_attention.jpg}&
\includegraphics[width=0.21\textwidth]{images/perobject_attn/GS_10_0_2_with_attention.jpg}&
\includegraphics[width=0.21\textwidth]{images/perobject_attn/GS_10_0_5_with_attention.jpg}\\

% \includegraphics[width=0.25\textwidth]{images/img_520} 
\rotatebox{90}{~~~~~~~~~~Events} &\includegraphics[width=0.21\textwidth]{images/perobject_attn/Events_10_0_0_with_attention.jpg}&
\includegraphics[width=0.21\textwidth]{images/perobject_attn/Events_10_0_1_with_attention.jpg}&
\includegraphics[width=0.21\textwidth]{images/perobject_attn/Events_10_0_2_with_attention.jpg}&
\includegraphics[width=0.21\textwidth]{images/perobject_attn/Events_10_0_5_with_attention.jpg}\\

\end{tabular}
}
\caption{Visualization of the attention map for each object using grayscale image and event frame as inputs, respectively.}
\label{fig:vis_attn}
\end{figure*}
